FixRoute: A Unified Logic and Numerical Tool for Provably Safe Internet Traffic Engineering

The performance of networks that use the Internet Protocol is sensitive to precise configuration of many low-level parameters on each network device. These settings govern the action of dynamic routing protocols, which direct the flow of traffic; in order to ensure that these dynamic protocols all converge to produce some 'optimal' flow, each parameter must be set correctly. Multiple conflicting optimization objectives, nondeterminism, and the need to reason about different failure scenarios make the task particularly complicated. We present a fast and flexible approach for the analysis of a number of such management tasks presented in the context of BGP routing. The idea is to combine {\em logical} satisfiability criteria with traditional {\em numerical} optimization, to reach a desired traffic flow outcome subject to given constraints on the routing process. The method can then be used to probe parameter sensitivity, trade-offs in the selection of optimization goals, resilience to failure, and so forth. The theory is underpinned by a rigorous abstraction of the convergence of distributed asynchronous message-passing protocols, and is therefore generalizable to other scenarios. Our resulting hybrid engine is faster than either purely logical or purely numeric alternatives, making it potentially feasible for interactive production use.

==> Makefile <==
###########################################################
#
# Makefile for LaTeX docs
#
# $Id: 
#

.SUFFIXES:
.SUFFIXES: .ps .dvi .tex

TEXINPUTS := .:${TEXINPUTS}
BIBINPUTS := .:${TEXINPUTS}

#all: eps dvi ps pdf # res
all: pdf
eps: fig obj

#PAPER=mosaic
PAPER=main

LATEX=pdflatex

ps:  $(PAPER).ps

pdf: $(PAPER).pdf
dvi: $(PAPER).dvi

obj: $(patsubst %.obj, %.eps, $(wildcard *.obj))
fig: $(patsubst %.fig, %.eps, $(wildcard *.fig))

res:
	make -C results
	make -C figs

clean:
	$(RM) *.aux *.log *.bbl *.blg *~ \#*\# *.toc *.idx *.out *.bak
	$(RM) $(patsubst %.tex, %.ps, $(wildcard *.tex))
	$(RM) $(patsubst %.tex, %.dvi, $(wildcard *.tex))
	$(RM) $(patsubst %.tex, %.pdf, $(wildcard *.tex))

distclean: clean
	$(RM) $(patsubst %.fig, %.eps, $(wildcard *.fig))
	$(RM) $(patsubst %.obj, %.eps, $(wildcard *.obj))

# only need -Ppdf if using CM fonts
#%.pdf: %.dvi $(wildcard *.bib)
#	dvips -Ppdf -G0 -t letter -o $*.tmp.ps $<
#	ps2pdf $*.tmp.ps $*.pdf
#	$(RM) $*.tmp.ps $*.dvi *.aux *.log *.bbl *.blg *.toc

%.pdf: $(wildcard *.tex) $(wildcard *.bib)
	$(LATEX) $*
	bibtex $*
	$(LATEX) $*
	if [ -e $*.toc ] ; then $(LATEX) $* ; fi
	if [ -e $*.bbl ] ; then $(LATEX) $* ; fi
	if egrep Rerun $*.log ; then $(LATEX) $* ; fi
	if egrep Rerun $*.log ; then $(LATEX) $* ; fi
	if egrep Rerun $*.log ; then $(LATEX) $* ; fi
	#dvips -t letter -z -Ppdf -G0 -D600 main.dvi -o main.ps
	#ps2pdf main.ps main.pdf

	$(RM) *.aux *.log *.bbl *.blg *.toc

%.ps: %.dvi
	dvips -Ppdf -G0 -tletter -o $@ $<
%.ps.gz: %.ps
	gzip -v9 $<

%.eps: %.obj
	tgif -print -eps $*

%.eps: %.fig
	fig2dev -L eps $< $@

